One-sided GRP Solver and Numerical Boundary Conditions for compressible fluid flows

In the computation of compressible fluid flows, numerical boundary conditions are always necessary for all physical variables at computational boundaries while just partial physical variables are often prescribed as physical boundary conditions. Certain extrapolation technique or ghost cells are often employed traditionally for this issue but spurious wave reflections often arise to cause numerical instability. In this paper, we associate this issue with the one-sided generalized Riemann problem (GRP) solver motivated by the accelerated piston problem in gas dynamics so that the extrapolation technique can be actually avoided. In fact, the compatibility arguments naturally requires to formulate the one-sided generalized Riemann problem and incorporate it into the numerical procedure of boundary conditions. As far as the interaction of nonlinear waves with physical boundaries, such a one-sided GRP solver shows significant effects, as numerical experiments demonstrate, on avoiding spurious wave reflections at the computational boundaries.

==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
 \usepackage{mathrsfs}
 \usepackage{subfigure}
 \usepackage{multirow}
 \usepackage{booktabs}
 \usepackage{caption}
 \usepackage[]{harpoon}
  \usepackage{mwe}
 \usepackage{hyperref}
  \usepackage{sidecap}
   \usepackage{diagbox}
   
 \captionsetup[figure]{labelfont={},labelformat={default},labelsep=period,name={\scriptsize{Fig}.}}

\usepackage{amsmath}
\numberwithin{figure}{section}

 \include{abbr-notation}

\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
 \newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}
\newtheorem{thm}{Theorem}[section]
\newtheorem{cor}[thm]{Corollary}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}
\theoremstyle{definition}
\newtheorem{defn}[thm]{Definition}
\theoremstyle{Assertion}
\newtheorem{asser}[thm]{Assertion}
\theoremstyle{remark}
\newtheorem{rem}[thm]{Remark}
\numberwithin{equation}{section}


% Sets running headers as well as PDF title and authors
\headers{One-sided GRP Solver and Numerical Boundary Conditions}{Jiequan Li and Qinglong Zhang}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{One-sided GRP Solver and Numerical Boundary Conditions for compressible fluid flows}%\thanks{Submitted to the editors DATE.}}
%\funding{This work was funded by the Fog Research Institute under contract no.~FRI-454.}

% Authors: full names plus addresses.
\author{Jiequan Li\thanks{Institute of Applied Physics and Computational Mathematics, Beijing;  Center for Applied Physics and Technology, Peking University, China; and State Key Laboratory for Turbulence Research and Complex System, Peking University, China.
 (\email{li\_jiequan@iapcm.ac.cn }).
 }
\and Qinglong Zhang\thanks{School of Mathematics and Statistics, Ningbo University,  China.  (\email{zhangqinglong@nbu.edu.cn}).
  }}
%\funding{  Email address:   li\_jiequan@iapcm.ac.cn (J. Li), zhangqinglong@nbu.edu.cn (Q. Zhang).}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

